Privacy-Preserving Obfuscation for Distributed Power Systems

This paper considers the problem of releasing privacy-preserving load data of a decentralized operated power system. The paper focuses on data used to solve Optimal Power Flow (OPF) problems and proposes a distributed algorithm that complies with the notion of Differential Privacy, a strong privacy framework used to bound the risk of re-identification. The problem is challenging since the application of traditional differential privacy mechanisms to the load data fundamentally changes the nature of the underlying optimization problem and often leads to severe feasibility issues. The proposed differentially private distributed algorithm is based on the Alternating Direction Method of Multipliers (ADMM) and guarantees that the released privacy-preserving data retains high fidelity and satisfies the AC power flow constraints. Experimental results on a variety of OPF benchmarks demonstrate the effectiveness of the approach.

==> experiments.tex <==


\section{Experimental Results}

This section reports on the obfuscation quality and ability to converge of PD-OPF. Additionally, the proposed method is compared with a centralized version that solves problem $P_{\RBL}$, thus admitting the presence of a centralized data curator. 
The experiments are performed on a variety of NESTA \cite{Coffrin14Nesta} benchmarks. 
Parameter $\epsilon$ is fixed to 1.0, the \emph{indistinguishability level} $\alpha$ varies from 0.01 to 0.1 in p.u. (i.e. 1 MVA to 10 MVA), and the \emph{fidelity level} $\beta$ varies from 10$^{-2}$ to 10$^{-1}$ (i.e. from 1\% to 10\% of the optimal cost difference). 
PD-OPF is limited to use 5000 iterations. 
All the models are implemented using PowerModels.jl~\cite{Coffrin:18} in Julia with nonlinear solver IPOPT~\cite{wachter06on}.

Choosing a penalty factor $\rho$ to drive convergenceis challenging~\cite{mhanna19adaptive}. Thus, the experimental routine adjusts $\rho$ dynamically, using the maximum primal and dual infeasibility values, $\epsilon_{p} = \max \bm{r}_p$ and $\epsilon_{d} = \max \bm{r}_d$, respectively (in spirit of~\cite{mhanna19adaptive}).
Higher values of $\rho$ encourage the satisfaction of the primal constraint, whiel lower values of $\rho$ shifts weight to the objectives and reduces the dual infeasibilities~\cite{mhanna19adaptive}. 
The heuristic adopted changes $\rho$ when the distance between $\epsilon_{p}$ and $\epsilon_{d}$ becomes too large:
\begin{align}
\rho &= \min\{(1+c)\rho, \overline{\rho} \}, &\mbox{ if } \epsilon_{p}  > c_t \epsilon_{d} \nonumber \\
\rho &= \max\{ \frac{\rho}{1+c}, \underline{\rho} \}, &\mbox{ if } \epsilon_{d}  > c_t \epsilon_{p}. \nonumber 
\end{align}
The scaling factor $c$ is set to $2\%$, the threshold parameter $c_t$ to $7.0$, and upper $\overline{\rho}$ and lower $\underline{\rho}$ bounds are respectively, $10^{6}$, and $5$.

To allow PD-POPF to restore primal feasibility, a \emph{feasibility boosting procedure} is implemented as follows. 
When the iteration counter 4500 iterations, if the maximum primal infeasibility is beyond $10^{-3}$, $\rho$ will be increased by: $\min\{(1+c)\rho, \overline{\rho} \}$.
We call this phase \emph{boosting}.
%regardless of the ratio-distance between the max primal and dual infeasibilities.

\subsection{Convergence Quality \& Runtime}
Table~\ref{tbl:conv1}
%-~\ref{tbl:conv2} 
presents the maximum primal infeasibility and dual infeasibility,
before the feasibility restoration procedure and after convergence (marked with $*$),
averaged over 50 instances on a variety of benchmarks.
Before the restoration procedure, max. primal infeasibilities mostly
stay at the order of $10^{-1}$ (p.u.),
and max. dual infeasibilities at the order of $1$ (p.u.).
With the boosting procedure, 
ADMM terminates with max. primal infeasibility up to target tolerance $10^{-3}$ for most benchmarks,
while sacrificing the max. dual infeasibility.

Figure~\ref{fig:conv_39} further shows the details of one run on the IEEE-39 benchmark. 
With a few iterations, both primal and dual infeasibilities stabilizes and reduces to approx $10^1$ to $10^{-1} $ order of magnitude (top-left),
and the generator cost stabilizes at around 2000 iterations (bottom-left).
After $90\%$ of the iterations,
since the primal infeasibility is still higher than the required tolerances $\epsilon_t=0.001$,
the coordination agent increases $\rho$ (bottom right), forcing all the agents to re-optimize with a higher penalty
for violations of coupling constraints.
Increasing $\rho$ degrades dual feasibility (top-right).

\begin{table}[h]
\centering
\setlength{\tabcolsep}{5pt}
\caption{Primal \& dual infeasibility, and Sim. runtime. $\alpha = 0.1, \beta = 0.1$. }
\resizebox{0.95\columnwidth}{!}{
\begin{tabular}{|l|rr|rr|r|}
\toprule
{} &  Primal &  Primal$*$ &  Dual &  Dual$*$ &   Time (min.) \\
\midrule
nesta\_case3\_lmbd      &        0.036 &                0.001 &      0.173 &              0.079 &   1.147 \\
nesta\_case4\_gs        &        0.023 &                0.001 &      0.092 &             13.953 &   2.110 \\
nesta\_case5\_pjm       &        1.580 &                0.015 &      3.094 &            380.243 &   3.501 \\
nesta\_case6\_c         &        0.203 &                0.001 &      0.835 &              7.088 &   2.607 \\
nesta\_case6\_ww        &        0.094 &                0.001 &      0.419 &              7.919 &   3.215 \\
nesta\_case9\_wscc      &        0.197 &                0.001 &      1.224 &              5.908 &   2.776 \\
nesta\_case14\_ieee     &        0.579 &                0.001 &      2.228 &             19.762 &   5.141 \\
nesta\_case24\_ieee\_rts &        0.293 &                0.006 &      1.276 &            540.403 &  11.157 \\
nesta\_case29\_edin     &        0.216 &                0.128 &      2.393 &           3027.724 &  38.686 \\
nesta\_case30\_as       &        0.386 &                0.001 &      1.685 &             15.223 &  12.592 \\
nesta\_case30\_fsr      &        0.416 &                0.001 &      2.215 &             14.001 &  10.738 \\
nesta\_case30\_ieee     &        0.621 &                0.001 &      2.831 &             37.137 &  11.167 \\
nesta\_case39\_epri     &        0.291 &                0.026 &      1.597 &           1849.358 &  15.273 \\
nesta\_case57\_ieee     &        0.584 &                0.001 &      2.951 &             62.776 &  19.614 \\
nesta\_case73\_ieee\_rts &        0.402 &                0.008 &      2.762 &            691.576 &  45.131 \\
nesta\_case118\_ieee    &        0.968 &                0.004 &      4.427 &            394.885 &  82.160 \\
nesta\_case189\_edin    &        3.214 &                0.017 &     14.780 &            871.245 &  86.908 \\
\bottomrule
\end{tabular} \label{tbl:conv1}
}
\end{table}


 
  
 
%\begin{table}[h]
%\scriptsize
%\centering
%\caption{Primal and dual infeasibility, and simulation runtime. $\alpha = 0.01, \beta = 0.01$. Average over 50 instances. }
%\begin{tabular}{lccc}
%\toprule
%Benchmark &  Primal Inf. (p.u.) &  Dual Inf. (p.u.) &  Total Time (min) \\
%\midrule
%nesta\_case3\_lmbd      &         0.00 &       0.02 &   0.05 \\
%nesta\_case4\_gs        &         0.00 &       0.14 &   0.91 \\
%nesta\_case5\_pjm       &         0.02 &     475.53 &   3.49 \\
%nesta\_case6\_c         &         0.00 &       0.65 &   0.87 \\
%nesta\_case6\_ww        &         0.00 &       1.24 &   2.09 \\
%nesta\_case9\_wscc      &         0.00 &       0.66 &   0.57 \\
%nesta\_case14\_ieee     &         0.00 &       4.98 &   4.56 \\
%nesta\_case24\_ieee\_rts &         0.01 &     652.90 &  10.32 \\
%nesta\_case29\_edin     &         0.11 &    2986.68 &  31.06 \\
%nesta\_case30\_as       &         0.00 &       0.68 &   6.27 \\
%nesta\_case30\_fsr      &         0.00 &       1.49 &   7.67 \\
%nesta\_case30\_ieee     &         0.00 &       5.80 &   7.19 \\
%nesta\_case39\_epri     &         0.04 &    1831.69 &  15.28 \\
%nesta\_case57\_ieee     &         0.00 &      17.82 &  13.27 \\
%nesta\_case73\_ieee\_rts &         0.01 &     706.56 &  40.35 \\
%nesta\_case118\_ieee    &         0.01 &     529.42 &  72.75 \\
%nesta\_case189\_edin    &         0.02 &     780.15 &  63.94 \\
%\bottomrule
%\end{tabular} \label{tbl:conv1}
%\end{table}


\begin{figure}[h]
	\centering
 	\includegraphics[width=.22\textwidth,valign=c]{results/iter-data/{{nesta_case39_epri_1_0.1-infeas}}}
 	\includegraphics[width=.22\textwidth,valign=c]{results/iter-data/{{nesta_case39_epri_1_0.1-infeaszoom}}}
	\includegraphics[width=.22\textwidth,valign=c]{results/iter-data/{{nesta_case39_epri_1_0.1-cost}}}
	\includegraphics[width=.22\textwidth,valign=c]{results/iter-data/{{nesta_case39_epri_1_0.1-rho}}}	
	\caption{Primal $\epsilon_{p}$ \& dual $\epsilon_{d}$ infeasibility (Full-scale: top left, $>4400$ iterations: top right), generator dispatch costs (bottom left), penalty $\rho$ (bottom right) on IEEE-39 bus. $\alpha =0.1$, $\beta=0.1$.
	The vertical dotted line marks the activation of the boosting procedure.} 
	\label{fig:conv_39}
\end{figure}

\subsection{Quality of Fidelity Restoration}
Figure~\ref{fig:opf} illustrates the loss in fidelity of the distributed mechanism. 
The box-plots report the percentage difference on the dispatch cost differences $\hat{\cO}$ between the original and obfuscated loads produced by 
the ADMM mechanism in percentages ($\%$) by
$100 \times \frac{\cO( \hat{\cO} - \cO(P_{\text{OPF}}({\bm{S}}^d)) }{ \cO(P_{\text{OPF}}({\bm{S}}^d)) }$, averaged over 50 instances.
Since the costs from ADMM may not necessarily be the true optimal costs, 
we also compared the optimal costs by running an AC-OPF routine on the 
obfuscated load (i.e. $P_{\text{OPF}}(\hat{S}^d)$).
\footnote{
Since the AC-OPF validation routine often require a higher level of numerical accuracy, 
the closest AC feasible loads (in L2 norm) at required numerical accuracy will be computed and used instead.}
The experimental results indicate ADMM manage to restore fidelity, even when beta is as small as
0.01 of the original dispatch costs with large dual infeasibility.

\begin{figure}[h]
	\centering
 	\includegraphics[width=.18\textwidth]{results/opf-diff/{{nesta_case39_epri_A0.01}}}
 	\includegraphics[width=.18\textwidth]{results/opf-diff/{{nesta_case39_epri_A0.1}}}\\
 	\includegraphics[width=.18\textwidth]{results/opf-diff/{{nesta_case57_ieee_A0.01}}}
 	\includegraphics[width=.18\textwidth]{results/opf-diff/{{nesta_case57_ieee_A0.1}}}
	\caption{IEEE 39 (top) \& IEEE 57 bus (bottom). Percentage Difference on the Dispatch Costs after ADMM and AC-OPF: $\alpha = 0.01$ (left), $0.1$ (right), $\beta=[0.1,0.01]$.} 
	\label{fig:opf}
\end{figure}

%\begin{figure}[h]
%	\centering
% 	\includegraphics[width=.18\textwidth]{results/opf-diff/{{nesta_case57_ieee_A0.01}}}
% 	\includegraphics[width=.18\textwidth]{results/opf-diff/{{nesta_case57_ieee_A0.1}}}
%	\caption{IEEE 57 bus. Percentage Difference on the Dispatch Costs after ADMM and AC-OPF: $\alpha = 0.01$ (left), $0.1$ (right), $\beta=[0.1,0.01]$.} 
%	\label{fig:opf_57}
%\end{figure}


\subsection{Quality of Load Demand Obfuscation}
Figure~\ref{fig:load} depicts the original loads (Orig.) from the IEEE-57 bus
systems, and compare them with the polar Laplace mechanism (Lap.) and the
ADMM solution. 
The loads are indeed different after the
Laplace mechanism and the ADMM post-processing.
With the final boosting procedure, most of the loads
are extremely close to the AC feasible solution.
For clarity reasons, we skip reporting those AC-feasible loads.

\begin{figure}[h]
	\centering
	\includegraphics[width=.25\textwidth,valign=t]{results/load-scatter-plot/{{Legend}}}
 	\includegraphics[width=.40\textwidth,valign=t]{results/load-scatter-plot/{{nesta_case57_ieee_8_0.1}}}
	\caption{Original loads distance from the Laplace and the PD-OPF Mechanisms on the IEEE-57 bus system.}% $\alpha = [0.01, 0.005]$}%, $\beta=0.1$.} 
	\label{fig:load}
\end{figure}



%The behavior is further validated by Figure~\ref{fig:orig-dist-39}-\ref{fig:orig-dist-57}, that shows the L2 distance between the ADMM, centralized validation, Laplace mechanisms and the original datasets over 50
%different instances. 
%ADMM return load solutions closely matching the restored loads by the validation process, indicating ADMM achieve high quality loads in terms of numerical accuracy (i.e. low primal infeasibility).
%Note that the Laplace loads typically give AC-infeasible power flows.

%\begin{figure}[h]
%	\centering
% 	\includegraphics[width=.20\textwidth,valign=c]{results/load-distance-to-original-plot/{{nesta_case14_ieee_A0.01}}}
% 	\includegraphics[width=.20\textwidth,valign=c]{results/load-distance-to-original-plot/{{nesta_case14_ieee_A0.1}}}
%	\caption{Load distance between Obfuscation Mechanisms and Original Dataset on IEEE-14, $\alpha =$ 0.01 (left), 0.1 (right), $\beta=[0.01,0.1]$. Average over 50 instances.} 
%	\label{fig:orig-dist-14}
%\end{figure}
%
%\begin{figure}[h]
%	\centering
% 	\includegraphics[width=.20\textwidth,valign=c]{results/load-distance-to-original-plot/{{nesta_case30_ieee_A0.01}}}
% 	\includegraphics[width=.20\textwidth,valign=c]{results/load-distance-to-original-plot/{{nesta_case30_ieee_A0.1}}}
%	\caption{Load distance between Obfuscation Mechanisms and Original Dataset on IEEE-30, $\alpha =$ 0.01 (left), 0.1 (right), $\beta=[0.01,0.1]$. Average over 50 instances.} 
%	\label{fig:orig-dist-30}
%\end{figure}

%\begin{figure}[h]
%	\centering
% 	\includegraphics[width=.20\textwidth,valign=c]{results/load-distance-to-original-plot/{{nesta_case39_epri_A0.01}}}
% 	\includegraphics[width=.20\textwidth,valign=c]{results/load-distance-to-original-plot/{{nesta_case39_epri_A0.1}}}
%	\caption{Load distance between Obfuscation Mechanisms and Original Dataset on IEEE-39, $\alpha =$ 0.01 (left), 0.1 (right), $\beta=[0.01,0.1]$. Average over 50 instances.} 
%	\label{fig:orig-dist-39}
%\end{figure}
%
%\begin{figure}[h]
%	\centering
% 	\includegraphics[width=.20\textwidth,valign=c]{results/load-distance-to-original-plot/{{nesta_case57_ieee_A0.01}}}
% 	\includegraphics[width=.20\textwidth,valign=c]{results/load-distance-to-original-plot/{{nesta_case57_ieee_A0.1}}}
%	\caption{Load distance between Obfuscation Mechanisms and Original Dataset on IEEE-57, $\alpha =$ 0.01 (left), 0.1 (right), $\beta=[0.01,0.1]$. Average over 50 instances.} 
%	\label{fig:orig-dist-57}
%\end{figure}

%\begin{figure}[h]
%	\centering
% 	\includegraphics[width=.20\textwidth,valign=c]{results/load-distance-to-original-plot/{{nesta_case189_edin_A0.01}}}
% 	\includegraphics[width=.20\textwidth,valign=c]{results/load-distance-to-original-plot/{{nesta_case189_edin_A0.1}}}
%	\caption{Load distance between Obfuscation Mechanisms and Original Dataset on Edinburg-189 bus, $\alpha =$ 0.01 (left), 0.1 (right), $\beta=[0.01,0.1]$. Average over 50 instances.} 
%	\label{fig:orig-dist-189}
%\end{figure}

\subsection{Quality of Privacy Loss Minimization}
We also compare the quality of our distributed ADMM algorithm against 
a centralized implementation on the privacy loss errors: $ \| \hat{\bm{S}}^d - \tilde{\bm{S}}^d \|^2$.
Figures~\ref{fig:lap-dist-39}-\ref{fig:lap-dist-189} show
the L2 distance between loads from the ADMM implementation and the centralized implementation~\cite{Fioretto:18b} 
against the Laplace solutions (averaged over 50 instances).
The load solutions returned by ADMM are comparable, and often extremely close to the centralized
mechanism when the dual infeasibilities are low, except for IEEE-39 with $\alpha=0.05$ 
when the final boosting mechanism is activated to regain primal feasibility by worsening dual feasibility.
The results indicate ADMM is a powerful distributed algorithm 
to achieve privacy and fidelity when even compared to a central optimization method.

  
%The centralized mechanism solves:
%\begin{align}	
%		\min
%			& \;\; \| \hat{\bm{S}}^d - \tilde{\bm{S}}^d \|^2
%			 \nonumber \\
%	\text{s.t.:}
%	& \quad \big| {\cO}({\bm{S}}^g) - \cO^*  \big| \leq \beta \cO^*
%		\nonumber  \\
%	&\quad \bm{S}^g \in \sC_{PF}({\hat{\bm{S}}}^d) \nonumber 
%\end{align}



%
%\begin{figure}[h]
%	\centering
% 	\includegraphics[width=.20\textwidth,valign=c]{results/load-distance-to-laplace-plot/{{nesta_case14_ieee_A0.01}}}
% 	\includegraphics[width=.20\textwidth,valign=c]{results/load-distance-to-laplace-plot/{{nesta_case14_ieee_A0.1}}}
%	\caption{Load distance between Obfuscation Mechanisms and Polar Laplace Dataset on IEEE-14, $\alpha =$ 0.01 (left), 0.1 (right), $\beta=[0.01,0.1]$. Average over 50 instances.} 
%	\label{fig:lap-dist-14}
%\end{figure}
%
%\begin{figure}[h]
%	\centering
% 	\includegraphics[width=.20\textwidth,valign=c]{results/load-distance-to-laplace-plot/{{nesta_case30_ieee_A0.01}}}
% 	\includegraphics[width=.20\textwidth,valign=c]{results/load-distance-to-laplace-plot/{{nesta_case30_ieee_A0.1}}}
%	\caption{Load distance between Obfuscation Mechanisms and Polar Laplace Dataset on IEEE-30, $\alpha =$ 0.01 (left), 0.1 (right), $\beta=[0.01,0.1]$. Average over 50 instances.} 
%	\label{fig:lap-dist-30}
%\end{figure}

\begin{figure}[h]
	\centering
 	%\includegraphics[width=.20\textwidth,valign=c]{results/load-distance-to-laplace-plot/{{nesta_case39_epri_A0.01}}}
 	%\includegraphics[width=.20\textwidth,valign=c]{results/load-distance-to-laplace-plot/{{nesta_case39_epri_A0.1}}}
	\includegraphics[width=.45\textwidth,valign=c]{results/load-distance-to-laplace-plot/{{nesta_case39_epri_A}}}
	\caption{L2 distance between ADMM/Centralized Mechanisms and Laplace Dataset on IEEE-39, $\alpha = [0.05, 0.1]$, $\beta=[0.01,0.1]$.} 
	\label{fig:lap-dist-39}
\end{figure}

\begin{figure}[pt]
	\centering
 	%\includegraphics[width=.20\textwidth,valign=c]{results/load-distance-to-laplace-plot/{{nesta_case57_ieee_A0.01}}}
 	%\includegraphics[width=.20\textwidth,valign=c]{results/load-distance-to-laplace-plot/{{nesta_case57_ieee_A0.1}}}
	\includegraphics[width=.45\textwidth,valign=c]{results/load-distance-to-laplace-plot/{{nesta_case57_ieee_A}}}
	\caption{L2 distance between ADMM/Centralized Mechanisms and Laplace Dataset on IEEE-57, $\alpha = [0.05, 0.1]$, $\beta=[0.01,0.1]$.} 
	\label{fig:lap-dist-57}
\end{figure}

\begin{figure}[pt]
	\centering
 	%\includegraphics[width=.20\textwidth,valign=c]{results/load-distance-to-laplace-plot/{{nesta_case189_edin_A0.01}}}
 	%\includegraphics[width=.20\textwidth,valign=c]{results/load-distance-to-laplace-plot/{{nesta_case189_edin_A0.1}}}
	\includegraphics[width=.45\textwidth,valign=c]{results/load-distance-to-laplace-plot/{{nesta_case189_edin_A}}}
	\caption{L2 distance between ADMM/Centralized Mechanisms and Laplace Dataset on Edin-189 bus, $\alpha = [0.05, 0.1]$, $\beta=[0.01,0.1]$.} 
	\label{fig:lap-dist-189}
\end{figure}

